Neural Multi-Task Learning for Teacher Question Detection in Online Classrooms

Asking questions is one of the most crucial pedagogical techniques used by teachers in class. It not only offers open-ended discussions between teachers and students to exchange ideas but also provokes deeper student thought and critical analysis. Providing teachers with such pedagogical feedback will remarkably help teachers improve their overall teaching quality over time in classrooms. Therefore, in this work, we build an end-to-end neural framework that automatically detects questions from teachers' audio recordings. Compared with traditional methods, our approach not only avoids cumbersome feature engineering, but also adapts to the task of multi-class question detection in real education scenarios. By incorporating multi-task learning techniques, we are able to strengthen the understanding of semantic relations among different types of questions. We conducted extensive experiments on the question detection tasks in a real-world online classroom dataset and the results demonstrate the superiority of our model in terms of various evaluation metrics.

==> overview.tex <==
The overall workflow of our end-to-end approach is shown in Figure  \ref{fig:framework}. Similar to \cite{li2020multimodal}, we efficiently process the large-volume classroom recordings by utilizing a well-studied voice activity detection (VAD) system to cut an audio recording into small pieces of utterances \cite{sohn1999statistical,zhang2012deep}. The VAD algorithm is able to segment the audio stream into segments of utterances and filter out the noisy and silent ones. Then, each utterance segment is fed into an ASR system for transcription. After that, we build a neural NLU model to extract the semantically meaningful information within each sentence and make the final question detection prediction. Please note that as an end-to-end framework, our model can be integrated seamlessly into a run-time environment in the practical usage.
